GraphPipe: Improving Performance and Scalability of DNN Training with Graph Pipeline Parallelism

Deep neural networks (DNNs) continue to grow rapidly in size, making them infeasible to train on a single device. Pipeline parallelism is commonly used in existing DNN systems to support large-scale DNN training by partitioning a DNN into multiple stages, which concurrently perform DNN training for different micro-batches in a pipeline fashion. However, existing pipeline-parallel approaches only consider sequential pipeline stages and thus ignore the topology of a DNN, resulting in missed model-parallel opportunities. This paper presents graph pipeline parallelism (GPP), a new pipeline-parallel scheme that partitions a DNN into pipeline stages whose dependencies are identified by a directed acyclic graph. GPP generalizes existing sequential pipeline parallelism and preserves the inherent topology of a DNN to enable concurrent execution of computationally-independent operators, resulting in reduced memory requirement and improved GPU performance. In addition, we develop GraphPipe, a distributed system that exploits GPP strategies to enable performant and scalable DNN training. GraphPipe partitions a DNN into a graph of stages, optimizes micro-batch schedules for these stages, and parallelizes DNN training using the discovered GPP strategies. Evaluation on a variety of DNNs shows that GraphPipe outperforms existing pipeline-parallel systems such as PipeDream and Piper by up to 1.6X. GraphPipe also reduces the search time by 9-21X compared to PipeDream and Piper.

==> contents/0_outline.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Outline
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


% Scenario 1: Our pp partitioner is better than existing ones
% \textbf{Outline}
% \begin{outline}[enumerate]
% \1 Introduction
% \1 Background
% % \1 Motivation [Optional]
% \1 System Design
%     \2 Overview
%     \2 Optimizer
%     \2 Scheduler (Runtime)
% % \1 Implementation [Optional]
% \1 Evaluation
%     \2 End-to-end result
%     \2 Search time
% \1 Related Work
% \1 Conclusion
%     \2 Or Limitations and Future Work
% \end{outline}

% Scenario 2: In-depth analysis of parallel stages
\textbf{Outline}
\begin{outline}[enumerate]
\1 Introduction
\1 Background: Pipeline Parallelism
% \1 Motivation [Optional]
\1 Parallel Stage: Key takeaways
    \2 Definition
    \2 Pipeline depth decrease with parallel stages ($P_l - P_p$)
    \2 Analytical form of memory footprint with parallel stages
        \3 Activation memory footprint coefficient of the first stage ($P_p$ vs. $P_l$)
        \3 Assume same microbatch size / partition for simpilicity
    \2 Analytical form of Fill/drain time with parallel stages
        \3 Bubble size ($(P_p - 1)(t_b + t_f)$ vs. $(P_l - 1)(t_b + t_f)$
        \3 Assume same microbatch size / partition for simpilicity
    \2 Non-trivial trade-off of having larger microbatch size
        % \3 Compare with parallel stage with same partition
        \3 $TPS_{max}$ decrease - with empirical plot (x-axis: microbatch size, y-axis: $TPS_{max}$)
        \3 Fill and drain time increase - with empirical plot (x-axis: microbatch size, y-axis: bubble size)
        \3 How this affects final objective ($T_{iter}$)
            \4 Variables: minibatch size, microbatch size, pipeline depth (or number of devices), $TPS_{max}$, partition, number of model branches
            \4 Plot $T_{iter}$ (x-axis: microbatch size, y-axis: $T_{iter}$)
        
\1 System Design
    \2 Overview
    \2 Optimizer
    \2 Scheduler (Runtime)
% \1 Performance analysis of PP configurations
%     \2 Number of branches ($B$)
%     \2 Pipeline depth ($P$)
%     \2 Number of stages ($S$)
%     \2 Number of devices ($N$)
%     \2 Microbatch size ($m_i$)
%     \2 Data-parallel degree ($d_i$)
%     \2 Parallel stages
%     \2 Per-stage microbatch size
% \1 Implementation [Optional]
\1 Evaluation
    \2 Memory footprint (linear vs. parallel)
        \3 X-axis: Minibatch size, Number of devices and branches
        \3 Challenge: activation memory is pressure with large number of devices
    \2 Fill/drain time (linear vs. parallel)
        \3 X-axis: Minibatch size, Number of devices and branches
    \2 End-to-end result (linear vs. parallel)
    \2 Contributing factor to improvement
        \3 Fill/drain time
        \3 $TPS_{max}$
    \2 Search time
\1 Related Work
\1 Conclusion
    \2 Or Limitations and Future Work
\end{outline}

\textbf{Key Points}
\begin{outline}[enumerate]
\1 How is GPP (or parallel stage) novel compared with existing works?
    \2 None of existing pipeline partitioners can do this
        \3 which is branch-aware partitioning to decrease pipeline depth
\1 Is the main claim (Parallel stage is important to have) valid? 
    \2 Our linear stage covers all possible partitions?
\1 What insight can we provide? 
\end{outline}

\newpage
% \begin{outline}[enumerate]
% \1 Per-stage microbatch size
% \1 Notion of parallel stages and scheduling for them
% \1 Dynamic scheduling of microbatches to reduce fill/drain period?
% \1 Communication scheduling to reduce memory pressure on earlier stages?
% \end{outline}

% Challenges:
% \begin{itemize}
%     \item For supporting non-sequential pipeline, we need to support cases where a microbatch needs to be sent to multiple receivers at different pipeline depths
% \end{itemize}


==> contents/past_versions/4_method_091423.tex <==
% TODO: figure: existing methods (linearization)

% problem formalization related symbols
\makeatletter
\DeclareRobustCommand{\cev}[1]{%
  {\mathpalette\do@cev{#1}}%
}
\newcommand{\do@cev}[2]{%
  \vbox{\offinterlineskip
    \sbox\z@{$\m@th#1 x$}%
    \ialign{##\cr
      \hidewidth\reflectbox{$\m@th#1\vec{}\mkern4mu$}\hidewidth\cr
      \noalign{\kern-\ht\z@}
      $\m@th#1#2$\cr
    }%
  }%
}

\newcommand{\sche}[2]{{#1}_{#2}}
\newcommand{\gpforward}[3]{\vec{{#1}}_{#2}^{(#3)}}
\newcommand{\gpbackward}[3]{\cev{{#1}}_{#2}^{(#3)}}

\begin{figure*}[t!]
    \centering
    \includegraphics[width=\textwidth]{fig/gpp_ex1.pdf}
    \caption{Graph Pipeline Parallelism vs. Sequential Pipeline Parallelism}
    \label{fig:gpp_example}
\end{figure*}

\section{Graph Pipeline Parallelism}
\label{sec:gpp}

\subsection{Background}
\label{subsec:spp}

Pipeline parallelism is a form of model parallelism with the goal of improving training throughput and device utilization. 
%Here, let us focus on conventional pipelining methods, which we collectively call sequential pipeline parallelism (\spp). 
A key idea of pipeline parallelism is to split both a DNN model and a training data batch into smaller pieces. Each piece of the DNN model is mapped to a stage and linked to other stages to form a pipeline.
Existing pipeline parallelism assumes that all stages form a sequential pipeline, which we refer to as {\em Sequential Pipeline Parallelism} (\spp). 
Given a device budget, we assign a subset of the devices to each stage, which executes the operators contained in the stage. 
We map each of the data batch pieces to a micro-batch and inject the micro-batches into the pipeline in cycles. In every cycle, the device subsets process different micro-batches and communicate their computation results to their next-in-line device subsets. 
From a micro-batch's perspective, it traverses the chain of the pipeline stages in a forward pass, and traverses the same chain in reverse in a backward pass, completing its processing.

Key elements of pipeline parallelism are thus as follows:
\begin{itemize}
    \item \textbf{Model Partitioning.} Viewing each forward (or backward) pass as a task, the workload for a task is determined by the amount of operators assigned to it. Model partitioning splits the set of operators of a DNN into multiple subsets and assigns them to stages with the goal of balancing the task workloads across the stages.
    \item \textbf{Device Assignment.} When multiple devices are assigned to a stage, we can apply data parallelism where a micro-batch is further split into pieces so that the devices can process them concurrently and aggregate their results. This extra dimension of parallelism offers an additional degree of freedom for balanced task execution.
    \item \textbf{Task Scheduling.} To maintain correctness of DNN training with pipeline parallelism applied, task scheduling ensures that the intricate data dependencies between all forward and backward tasks are respected.
\end{itemize}


% processing the micro-batches (micro-batches) and pipeline them over pipeline stages. Each pipeline stage is defined as a set of devices running a partition of a DNN model. Data dependencies of model partition rules data dependencies between stages. In every cycle, each device processes a different micro-batch and pass their result onto the next device, resulting in a micro-batch traverses the chain of pipeline stages in a forward pass. Likewise, the corresponding backward pass also traverses the chain in reverse. As in \SOO{FIGURE ?}, it significantly reduce device idle time in warm-up phase of every training iteration compared with the case with no pipeline parallelism.


% Mention the possibility of data parallelism


% \ZJ{The term generalized pipeline parallelism has been used in the PipeDream paper, so we cannot overload that term. My suggestion is to call our work graph pipeline parallelism (GPP), and refer to existing approach sequential pipeline parallelism (SPP).}

% Let us begin by providing a brief overview for parallel DNN training and formalizing the problem setup of this work. We then introduce our novel parallel DNN training strategy, which we call {\em graph pipeline parallelism} (\gpp), and present a high-level comparison between \gpp and existing sequential pipeline parallelism (\spp).

% \paragraph{Background.}
% % DNN training
% A DNN describes a set of operators applied to input data as well as their execution order to produce output data. Training a DNN involves fine-tuning all parameters associated with its operators using a dataset, which usually consists of input-output pair samples. Training progresses in iterations. In each, we pass the input of $B \geq 1$ (mini-batch size) samples through a DNN to produce $B$ output estimations, evaluate the quality of the estimations with respect to the output of the $B$ samples, and update the parameters based on the evaluation. We refer to the computation of the input data as a forward pass, and the calculation of the gradients required to update the parameters as a backward pass.

% % parallel DNN training
% Multiple devices can be used to parallelize DNN training. Distinct devices take on a portion of the total work involved, compute their shares simultaneously, and communicate their computations with each other as needed. Various parallelization techniques have been developed. Of many, let us describe two techniques primarily employed in this work.

% % data parallel
% \emph{Data parallelism}. Multiple devices have an identical copy of a DNN. A batch of training data is split across the devices and each device performs the computation using the partial input data assigned. As each device has access to a subset of each mini-batch and the gradient calculation is performed with respect to the entire mini-batch, the devices communicate with each other to update the parameters.

% % pipeline parallel
% \emph{Pipeline parallelism}. A DNN is partitioned into multiple pieces, corresponding to pipeline stages, which have data dependencies between them. Distinct devices assigned to the stages are pipelined according to the dependencies. A batch of training data is split into smaller batches (micro-batches) and injected into the pipeline. In every cycle, the devices each process a different micro-batch and pass their result onto the next device, resulting in a micro-batch traverses the chain of pipeline stages in a forward pass. Likewise, the corresponding backward pass also traverses the chain in reverse.

% % combination of the two
% Combining different parallelization techniques is possible, and often desirable. Suppose we have 16 devices to employ. We can split a DNN model into four pipeline stages and assign four devices to each stage. This combination can help reduce the memory footprint for each model piece through pipeline parallelism so that a single device can store a piece, and also enable fast processing (owing to concurrent execution by four devices) of the piece per data sample through data parallelism.

\subsection{High-Level Distinction of \gpp}
\label{subsec:high-level-gpp}

Now, let us present a high-level distinction of \gpp in comparison with \spp. Figure~\ref{fig:gpp_example} illustrates how \gpp partitioner and scheduler are different from \spp given the same DNN to train.

\spp partitioner first linearizes the operators in a way that respects their data dependencies, and then partitions the linearized DNN into pipeline stages. The relationships between stages are simple: only one predecessor and one successor for each stage. The execution order of stages is thus strictly sequential.

In stark contrast, \gpp partitioner preserves its topology while partitioning the DNN into pipeline stages. The relationships between stages are \emph{graphical}. The execution order of stages can be thus more general compared to \spp. This topology-aware model partitioning and pipeline stage execution provides \gpp a clear advantage: concurrent execution of stages that are computationally-independent.

%Next, let us compare \gpp scheduler with \spp scheduler.
With topology-preserved stage partitions, \gpp scheduler parallelizes pipeline stages that are computationally-independent to each other (e.g., $S_1, S_2, S_3$) while \spp scheduler assumes all stages are sequential. For example, stages $S_1$ and $S_2$ do not have data dependencies in the original DNN (not in the linearized DNN though), yet \spp processes them sequentially. On the other hand, \gpp processes stages $S_1, S_2, S_3$ \emph{concurrently} as they do not have data dependencies. This leads to a shorter warm-up and cool-down phase. As a result, \gpp achieves a shorter training iteration time over \spp.

For such parallelism, it is important that \gpp partitioner is aware of DNN topology and in fact exploits it to maximize parallelism while \spp does not. For example, \gpp generates parallel stage partitions (e.g., $S_1, S_2, S_3$) while \spp unexpectedly creates dependency between $S_2$ and $S_3$ by blindly partitioning DNN into stages. 

%\gpp preserves the topology of the DNN in partitioning pipeline stages, and in fact exploits it, while \spp does not. This leads to (a) a shorter initialization phase until the pipeline becomes full; and (b) a shorter execution time while the pipeline is full. As a result, \gpp achieves a shorter training iteration time over \spp.

Figure~\ref{fig:gpp_example} assumes that the micro-batch sizes across stages are identical for simplicity. However, we design \gpp in such a way that it allows for \emph{different} micro-batch sizes across distinct stages, while \spp does not. Granted, this allowance complicates scheduling of forward and backward passes as different stages deal with varied micro-batch sizes. But this added complexity may prove worthwhile in certain cases. Depending on numerous factors, such as hardware, operator kernel implementations, compute efficiencies of different operator sets may demonstrate varied scalabilities with respect to the number of data samples. This scalability heterogeneity can be further leveraged by using different micro-batch sizes across distinct stages in order to balance the task execution times in a fine-grained manner.

\subsection{Performance Discussion}
\label{sec:high-perf}

Let us reason about conditions for high performance pipelines in distributed DNN training, and advocate that \gpp is a superior approach toward meeting such conditions over \spp.
% Let us step back from the details of \gpp for a moment and reason about the conceptual framework for high performance pipelines in the context of parallel DNN training.

\paragraph{Keys to High Pipeline Performance.} Key aspects instrumental to high pipeline performance are: (a) load balancing, (b) compute efficiency, and (c) warm-up.
\begin{itemize}
    \item Load balancing across stages alleviates the burden of the bottleneck stage, thus is crucial, as pipeline performance hinges upon the straggler. The amounts of workloads need to be spread across stages in a way that no single stage has a much higher workload than the others.
    \item Compute efficiency of each operator affects system throughput, i.e., number of samples processed per second. It is common to increase (micro-)batch size to increase operational intensity, thus improve compute efficiency.
    \item Warm-up is the initial phase of the pipeline operation during which tasks are being injected into the pipeline until it becomes full so that all devices can be utilized concurrently. Some devices are left idle doing no useful work during warm-up, so it is desirable to curb it.
\end{itemize}

These aspects look seemingly independent at first glance. But upon close inspection, especially in the context of parallel DNN training, we can discover that there exists one design variable that ties them all: pipeline depth.

\paragraph{Pipeline Depth.}
% In other words, it is the longest distance between any two stages when the distance between two stages is the length of the shortest path between them.
We define \emph{pipeline depth} as maximum number of sequential pipeline stages for a given stage graph. The relationship between pipeline depth and warm-up is clear: the shorter the pipeline depth, the shorter the warm-up phase (in terms of cycles). To curb warm-up, the strategy can be devised so as to reduce pipeline depth.

\paragraph{Memory Usage.} Recall that the need for pipeline parallelism arises from the recent trend that the sizes of DNNs are ever-growing. While device memory usage is not the primary performance metric, it still is central to the problem.

All else being equal, lower device memory usage provides us the \emph{flexibility} in (a) splitting a given DNN into a better partition that otherwise would not have been possible due to memory constraints (better load balancing); and (b) increasing micro-batch size, thus increasing operational intensity of each operator and eventually, system throughput.

\paragraph{Pipeline Depth and Memory Usage --- Connection.}
There exists a close connection between pipeline depth and device memory usage. Let us establish it, thereby demonstrating the case for pipeline depth being the integral design variable that impacts all three key aspects of high pipeline performance.

The pipeline operation in distributed DNN training is marked by its bi-directional nature. A stage is said to fully-process a micro-batch when the micro-batch passes through a pipeline stage once in the forward pass, and again in the backward pass in the opposite direction. An inevitable delay occurs in between. As the two passes are computationally-\emph{dependent}, the activation result of the forward pass needs to be stored temporarily until after the backward pass is complete. This storage requirement leads to \emph{activation} memory usage.

The delay between a pair of forward and backward passes is longest for the first stage and shortest for the last stage, and this delay discrepancy increases in proportion to pipeline depth. The whole point of pipelining is to keep all devices busy, so there is a constant stream of micro-batches being injected into the pipeline. This stream creates a buildup of micro-batches yet to be fully-processed in each stage, which we call \emph{in-flight} micro-batches. Also, the amount of buildup for a stage increases in proportion to the associated delay. As a result, activation memory usage increases monotonically toward early stages along the pipeline.

On the other hand, \emph{weight} memory usage depends entirely on the amount of operators in a stage regardless of its position in the pipeline. These two types of memory usage constitute total memory pressure.

It is then clear to see how pipeline depth is closely related to device memory usage. As pipeline depth increases, \emph{activation} memory pressure tends to increase (in spite of it falling disproportionately upon early stages of the pipeline), and in contrast, \emph{weight} memory pressure tends to decrease because the fixed total amount of operators in a DNN is spread across a larger number of stages. Total memory pressure falling upon a single stage being the sum of the two, there exists a trade-off and pipeline depth plays a crucial role in weighing it.

\paragraph{Advantages of \gpp over \spp.} We established that pipeline depth impacts all three key aspects of high pipeline performance, so let us demonstrate how \gpp reduces pipeline depth to improve performance in comparison to \spp.

Recall that a complete sequence of the stages is required in \spp. This requirement implies that the pipeline depth of \spp is always equal to the number of stages. In stark contrast, \gpp allows directed graph-like dependencies between the stages. As a direct result, \gpp can generate a strategy where the pipeline depth is in fact less than the number of stages.

All else being equal (assuming identical model partition and device assignment for fair comparison), \gpp being capable of achieving shorter pipeline depth has two main implications. First, it means less warm-up. Under the assumptions, the smaller number of warm-up cycles translates directly into less warm-up time. Second, it means lower activation memory usage. The same model partition leads to the same weight memory usage for both strategies. Thus, the total memory usage is smaller for \gpp. This advantage expands the range of micro-batch sizes from which \gpp can choose, thus offers the flexibility in setting micro-batch sizes more liberally to generate a superior strategy by either choosing a larger micro-batch size (improved compute efficiency) or better exploiting scalability heterogeneity across stages.

% \paragraph{High-Level Distinction of \gpp.} Let us highlight the two-fold distinction between \gpp and all other existing pipeline methods, which we collectively call sequential pipeline parallelism (\spp), for the time being from an operational perspective only. We defer discussion of its performance implications to the next sections.

% To begin with, \gpp allows for \emph{different} micro-batch sizes $b_i$'s across distinct stages, while \spp does not. This allowance complicates scheduling of forward and backward passes as we can see in \textit{C5}. In this regard, using the same micro-batch size across all stages in \spp is desirable for its simplicity. But we will demonstrate that it leaves on the table potential performance improvements worth the added complexity.

% More importantly, note \textit{C2} and \textit{C5}, which concern pairs of stages. \textit{C2} states that unless there exists $(u,v) \in \m{E}_C$ such that $u \in \m{G}_i$ and $v \in \m{G}_j$, a pair of stages $(S_i, S_j)$ need \emph{not} be an element of $\m{E}_S$. Also, \textit{C5} states that \emph{no} scheduling requirement is imposed on a pair of stages $(S_i, S_j) \notin \m{E}_S$. Combined, these fine details of \textit{C2} and \textit{C5} have an important implication, which becomes clear in contrast with \spp.

% \spp necessitates that a complete sequence of stages be established, which in turn specifies the execution order between any given pair of stages. This execution order between stages $S_i$ and $S_j$ needs to be respected whether or not there exists $(u,v) \in \m{E}_C$ such that $u \in \m{G}_i$ and $v \in \m{G}_j$. This requirement by design enforces any micro-batch to be processed exclusively by only one stage at a time.

% The absence of such requirement in \gpp creates substantial room for improvement as a micro-batch can be processed concurrently by multiple stages.\footnote{A note of caution is in order. This form of concurrent processing is different from that in data parallelism where multiple devices perform the same set of operators concurrently. Here, multiple devices perform distinct sets of operators on the same micro-batch concurrently.} This mode of pipelining is certainly unconventional. Yet it is viable in parallel DNN training because tasks being pipelined can be made independent depending on how a DNN model is partitioned.

% In the following sections, we will demonstrate that this two-fold distinction opens up the possibility of attaining superior performance employing \gpp over \spp. We will first present key functional elements of \gpp (\S\ref{sec:key-gpp-elements}) in further detail. We will then discuss main pillars of high pipeline performance (\S\ref{sec:high-perf}) and finally piece them together so as to highlight the novelty of \gpp over \spp (\S\ref{sec:in-depth}).

% \paragraph{} Let us now present \gpp in greater detail. We will begin by laying out major functional elements of \gpp in \S\ref{sec:key-gpp-elements}. We will then discuss main pillars of high pipeline performance and key design variables for pipeline parallelism to realize them in \S\ref{sec:high-perf}. With the details in place, we will conclude by mapping the functional elements of \gpp to the key variables, conducting an in-depth comparison of \gpp and \spp in \S\ref{sec:in-depth}.


% CONTENT MOVED SOMEWHERE ELSE
% \subsection{Functional Elements of \gpp}
% \label{sec:key-gpp-elements}

% % Now, let us discuss in detail each of four key components of training strategy $\m{G}_S = (\m{V}_S, \m{E}_S)$.
% Recall each stage is a four-element tuple: $S_i = \langle \m{G}_i, b_i, \m{D}_i, \Pi_i \rangle$. Each of these elements performs a unique function and is on its own pivotal to achieving high performance.

% \paragraph{Model Partitioning.} Viewing each of forward and backward passes as a task, the workload for a task is determined by the amount of operators assigned to the task. Model partitioning splits the set of operators of a DNN model into multiple subsets and assigns them to stages in such a way that the task workloads are well-balanced across the stages so as to optimize the performance of interest in a min-max fashion (see (\ref{opt:objective})). But note that model partitioning cannot achieve it single-handedly. It is one thing to balance workloads, and it is another to execute them to achieve the goal.

% \paragraph{Micro-Batch Size Adjustment.} Various types of operators constitute a DNN model. Depending on numerous factors, such as device hardware technologies, driver and library implementations, compute efficiencies of different operators demonstrate varied scalabilities with respect to the number of data samples. This heterogeneity is exploited through using different micro-batch sizes across distinct stages in order to balance the task execution times in a fine-grained manner.

% \paragraph{Device Assignment.} The number of stages does not need to be equal to the number of devices. When multiple devices take on a stage, data parallelism can be applied. This extra dimension of parallelism in addition to pipeline parallelism offers an extra degree of freedom in achieving efficient and balanced task execution. Note that all three functions above --- distribution of task workloads, fine-grained adjustment of compute efficiencies, and allocation of resources --- need to be \emph{jointly} optimized to achieve the goal of 
% (\ref{opt:objective}). This joint optimization is performed by the \emph{partitioner} of \gpp (see \S\ref{sec:partitioner}).

% \paragraph{Task Scheduling.} For correctness of pipeline parallelism, task scheduling ensures that all data dependencies governed by \textit{C4--C5} are respected. More importantly, it serves the function of memory management. We defer in-depth discussion of this instrumental function to \S\ref{sec:high-perf} and that of its optimality to \S\ref{sec:scheduler} where the \emph{scheduler} of \gpp is presented. For now, let us remark that task scheduling is primarily aimed at ensuring fundamental feasibility of any pipeline-parallel strategy by meeting the memory constraint of (\ref{opt:constraint}) so that all three previous functions can be geared toward achieving performance (\ref{opt:objective}).

% Memory usage consists of two parts: activation-related memory usage (e.g., activations and activation gradients), and parameter-related memory usage (e.g., model parameters, parameter gradients, and optimizer information). Given a stage $S_i$, the memory usage is
% \[
% M(S_i) = \mathrm{inflight}(\Pi_i) \cdot A(\m{G}_i, \m{D}_i) + c_W \cdot W(\m{G}_i, \m{D}_i),
% \]
% where $c_W$ is a constant coefficient once the training method is determined. $\mathrm{inflight}(\Pi_i)$ is the number of in-flight activation samples to be cached in the device, which is calculated by
% \begin{align*}
%     \mathrm{inflight}(\Pi_i) 
%         =& m_i \cdot \max_{x=1}^{|\Pi_i|} (\text{\# of forward microbatch before }x \\
%         &- \text{\# of backward microbatch before }x ).
% \end{align*}

% \paragraph{Micro-Batch Size: Is Larger Always Better?} Is it always desirable to increase micro-batch sizes to achieve highest compute efficiency possible? There are a few more nuanced trade-offs to consider, as although increasing micro-batch sizes mostly impacts compute efficiency, it also impacts other aspects of pipelining in indirect ways.

% \paragraph{Warm-up and Cool-down Cycles.} We have also discussed the relationship between warm-up/cool-down phases and pipeline depth. In this section, let us delve into this matter also taking an analytical view. Explain: $(P_p - 1) (t_b + t_f)$ v. $(P_l - 1)(t_b + t_f)$





% \subsection{Novelty of \gpp over \spp}
% \label{sec:in-depth}

% So far we have examined the key functions of \gpp in \S\ref{sec:key-gpp-elements} and laid out the conceptual framework of high performance pipelines in the context of parallel DNN training in \S\ref{sec:high-perf}. Now let us demonstrate the novelty of \gpp over \spp by showing how the main pieces of \gpp fit into the framework.

% We have shown that pipeline depth is a key design variable that impacts all aspects of pipeline performance. We now demonstrate that \gpp is better positioned to adjust it compared to \spp. Let us consider a hypothetical scenario where \gpp and \spp are employed to parallelize the same DNN model on the same device budget. To make our discussion simple, let us further assume that the model is split into an identical partition of stages and assignment of devices. Then the only main decision left in devising a strategy is to specify $\m{E}_S$ that establishes dependencies between the stages.

% A complete sequence of the stages is required in \spp. This requirement implies that the pipeline depth of \spp is always equal to the number of stages. In stark contrast, \gpp allows directed graph-like dependencies between the stages. As a direct result, \gpp can generate a strategy where the pipeline depth is in fact less than the number of stages.

% All else being equal (model partition and device assignment identical as assumed), the shorter pipeline depth of \gpp has two implications. First, it means less warm-up. Under the assumptions, the smaller number of warm-up cycles translates directly into less warm-up time. Second, it means lower activation memory usage. The same model partition leads to the same weight memory usage for both strategies. Thus, the total memory usage is smaller for \gpp. This advantage expands the range of micro-batch sizes from which \gpp can choose, thus offers the flexibility in setting micro-batch sizes more liberally to generate a superior strategy by either choosing a larger micro-batch size (improved compute efficiency) or better exploiting scalability heterogeneity across stages.

% \paragraph{Remarks.} It is time we leave cautionary remarks. It bears repeated emphasis that shorter pipeline depth provides the flexibility, not certainty, in setting key design variables critical to superior performance. It merely expands the strategy search space from which pipeline parallelism can potentially benefit. The contribution of this work is that we develop \gpp so as to explore this expanded search space that \spp cannot.

% It is also worth noting that it is not the case that \gpp always leads to a shorter pipeline depth over \spp, and also it is not the case that a shorter pipeline depth always leads to a better performance. The first is easy to see: consider a DNN model that consists of a single long sequence of operators. \gpp and \spp would generate the same strategy. As we will see in \S\ref{sec:evaluation}, DNN models for which \gpp outperforms \spp exhibit certain topological characteristics. The second needs elaboration.

% Other than design variables, there are also fixed external factors, such as DNN model $\m{G}_C$ and mini-batch size $B$, which are important considerations. Let us look into each.

% \textit{When shorter pipeline has little impact.} Suppose $\m{G}_C$ has operators that involve large numbers of weights and small numbers of activations. Recall that our discussion on shorter pipeline depth being a conduit for better memory management has relied on the assumption that activation memory usage is comparable to weight memory usage. What if it is not the case as in supposed $\m{G}_C$? As pipeline depth increases, weight memory usage decreases as the model weights are spread across more stages, at the cost of increased activation memory usage. But the cost can be negligible with a large ratio of weights to activations inherent in $\m{G}_C$, implying that a shorter pipeline may not necessarily be a better choice.

% \textit{When shorter pipeline can backfire.}
% Suppose $B$ is small. During DNN training, the model parameters are updated at the end of each iteration, and the updated ones need to be used at the beginning of the next iteration. This process implies that some devices, even after they finish their tasks, need to remain idle for a while until all other devices finish theirs. It is the phase of cool-down, symmetric to warm-up. Let us refer to the aggregate of warm-up and cool-down cycles as pipeline bubbles. Intuitively, the ratio of full pipeline cycles to bubbles in an iteration is an important proxy to performance: the higher the better. Examining pipeline performance through the lens of this ratio, setting larger micro-batch sizes to achieve higher compute efficiencies, enabled by a shorter pipeline depth, can backfire. With fixed $B$, the number of micro-batches is inversely proportional to the micro-batch size. With fewer micro-batches, the ratio dwindles and as a result the performance can deteriorate.


% As we have seen in the discussions of pipeline performance and in-depth comparisons of \gpp and \spp, there are numerous trade-offs to weigh simultaneously, and it is thus challenging to draw conclusions universally true in parallel DNN training and build on them to design training strategies. Facing this challenge, we propose an optimization algorithm that computationally weighs key trade-offs and efficiently generates a good \gpp strategy. The overview and details are to follow.





%% OUTDATED
% \paragraph{Improved training throughput.} \gpp can generally achieve better training performance than \spp by using non-sequential stage graphs and supporting per-stage microbatch sizes. In particular, the stage graphs supported by \gpp can be arbitrary DAGs, which enables a larger and more comprehensive search space and includes the linear stage graphs considered by \spp as special cases. This generalization allows \gpp to discover novel non-sequential pipeline parallelism strategies that outperforms \spp. Second, the per-stage microbatch size design enables \gpp to leverage performance heterogeneity across layers in a DNN model and allows \gpp to opportunistically optimize GPU utilization for specific stages while maintaining a relatively low memory requirement.

% \paragraph{Reduced memory requirement.} In addition to improving training throughput, \gpp also reduces memory requirement for pipeline parallel training compared to \spp. As shown in Figure xxx, both \spp and \gpp require keeping the intermediate results for in-flight microbatches for backward propagation. By leveraging the graph structure of a DNN model, \gpp can substantially reduce the pipeline depth and peak memory usage compared to \spp.

% \subsection*{Original version}
% We use \textit{cycle} as the basic time unit, i.e., a stage of microbatch size $m$ takes $m$ cycles to process a minibatch. Therefore, the time for a cycle, i.e., time per sample(TPS), is bounded by the slowest stage.

% Given the batch size $B$, the input computation graph $G_C = (V_C, E_C)$, and a device topology $D = (V_D, E_D)$:
% \begin{itemize}
%     \item We define a stage $s_i$ as a tuple $(g_i, m_i, d_i)$ where $g_i \subseteq V_C$ is the subgraph $s_i$ is responsible for, $m_i$ is the microbatch size of $s_i$, and $d_i$ is the set of devices $s_i$ uses;
%     \item There are $B/m_i$ forward and backward microbatches. We define a schedule $\sche{S}{i}$ for stage $s_i = (g_i, m_i, d_i)$ as a sequence of the $2B/m_i$ microbatches where the $j$-th forward microbatch should come before the $j$-th backward microbatch. This sequence determines the execution order of the microbatches within a stage, i.e., we should consider a data dependency between two consequent microbatches in this sequence.
%     \item We define a generalized pipeline parallelism strategy as a set of stages $P=\{s_i=(g_i, m_i, d_i)\}_i$ and a set of schedules $S=\{\sche{S}{i}\}_{i=1}^{|P|}$ s.t. $\{g_i\}_{i=1}^{|P|}$ is a partition of $V_C$, $\{d_i\}_{i=1}^{|P|}$ is a partition of $V_D$, and all the data dependencies are not violated.
% \end{itemize}

% \paragraph{Stage Graph}
% With a computation graph $G_C$ and a set of stages $P$, we define the stage graph $G_S = (V_S, E_S)$ where each node denotes a stage: $V_S = \{g_i\}_{i=1}^{|P|}$, and each edge denotes a data dependency between stages: $E_S = \{ (g_i, g_j) \mid g_i, g_j \in V_S, \exists o_x \in g_i, o_y \in g_j, s.t. (o_x, o_y) \in V_C \}$. In this work, we focus on strategies that derive acyclic stage graphs.



==> contents/past_versions/6_scheduler_ver1.tex <==
\section{Scheduler}
\label{sec:scheduler}

Static scheduling performs two functions. One is to ensure operational correctness of graph pipeline parallelism by meeting the data dependency requirements between all forward and backward passes within a stage (\textit{C4} in \S\ref{sec:gpp}) and those across distinct stages (\textit{C5} in \S\ref{sec:gpp}). The other is to ensure that the device memory constraint of (\ref{opt:constraint}) is not violated.

\begin{algorithm}[th!]
	\small
	\caption{Static Scheduler} \label{alg:microbatch-scheduling}
	\textbf{Input}: Stage subgraphs $\{\m{G}_i\}$, micro-batch sizes $\{b_i\}$, device allocations $\{\m{D}_i\}$ \\
	\textbf{Output}: Schedules $\{\Pi_i\}$\\
	\begin{algorithmic}[1]
            \For {$S_i \in \m{V}_S$}
                \If {no micro-batch schedule is specified for $S_i$}
                    \State \Call{ScheduleStages}{$S_i$}
                \EndIf
            \EndFor
            \Function{ScheduleStages}{$S_i$}
                \For {$\langle S_i, S_j \rangle \in \m{E}_S$}
                    \If {no micro-batch schedule is specified for $S_j$}
                        \State \Call{ScheduleStages}{$S_j$}
                    \EndIf
                \EndFor
                \State $\Pi_i \gets$ \Call{ScheduleTasks}{$b_i, \m{D}_i, \{\Pi_j \mid \langle S_i, S_j \rangle \in \m{E}_S\}$}
            \EndFunction
	\end{algorithmic}
\end{algorithm}

Algorithm~\ref{alg:microbatch-scheduling} describes static scheduling in detail. As input, it takes a configuration of model partition $\{ \m{G}_i \}$, micro-batch sizes $\{ b_i \}$, and device assignment $\{ \m{D}_i \}$. As output, it produces the set of static schedules $\{ \Pi_i \}$ of all forward and backward passes for all stages. As shown in Figure~\ref{fig:system-overview}, the input is fed by the partitioner (described in \S\ref{sec:partitioner}), and the output is returned back to it to indicate feasibility of the input.

Function \textsf{ScheduleStages} in Algorithm~\ref{alg:microbatch-scheduling} performs recursive search over stage graph $\m{G}_S = (\m{V}_S, \m{E}_S)$. It starts by first specifying a schedule for the last stage. Then for $\langle S_i, S_j \rangle \in \m{E}_S$, it traces back the directed edges in $\m{E}_S$ of $\m{G}_S$ in reverse and specifies schedules for stages $S_i$ until a schedule for the first stage is finally specified. The reason for backward traversal is that computing the activation memory usage, and thus the total usage, for a stage $S_i$ requires complete schedule information of subsequent stages $S_j$ for $\langle S_i, S_j \rangle \in \m{E}_S$.

Function \textsf{ScheduleTasks} in Algorithm~\ref{alg:microbatch-scheduling} specifies a schedule of all forward and backward tasks within a stage. Combined with \textsf{ScheduleStages}, it ensures the data dependency requirements \textit{C4--C5} in \S\ref{sec:gpp}. We consider three different methods of scheduling forward and backward passes within a stage: greedy, $k$F$k$B, and 1F1B.

\begin{figure}
    \centering
    \includegraphics[width=\columnwidth]{fig/1F1BvsnFnB.pdf}
    \caption{1F1B vs. $k$F$k$B}
    \label{fig:1f1b_nfnb}
\end{figure}

\paragraph{Static Scheduling Performance.} In evaluating the performances of different methods, we can take memory usage or time complexity perspectives. Let us focus on the memory usage criterion, as static scheduling is not directly related to the objective  (\ref{opt:objective}) of the optimization problem, but rather closely-related to the memory constraint (\ref{opt:constraint}). Also, whenever we discuss performance, we can reason about the \emph{optimality} aspect of it. In words, a schedule can be said optimal in terms of memory usage when no other schedule can achieve a better memory usage pattern. The formal definition is as follows.

\textit{Definition (Optimal Schedule).} Let $S_1, \dots, S_{|\m{V}_S|}$ be a topological order of stages in $\m{V}_S$. A schedule $\{\Pi_i\}$ is optimal if for any other schedule $\{\Pi'_i\}$ and a stage $S_i$, $\textsf{in-flight}(\Pi'_i) < \textsf{in-flight}(\Pi_i)$ implies $\textsf{in-flight}(\Pi'_j) > \textsf{in-flight}(\Pi_j)$ for some $j > i$, where $\textsf{in-flight}(\Pi_i)$ is the maximum number of micro-batches to be resolved for stage $S_i$ at some moment according to schedule $\Pi_i$.

Now let us visit each method and discuss its performances. First, the greedy method performs grid search to find the best micro-batch sizes for all stages. It also attempts to schedule each backward pass as early as possible within a stage in order to resolve in-flight micro-batches fast. We can prove that the greedy method produces an optimal schedule, and defer the proof and the details of the implementation to Appendix~\ref{sec:greedy-proof}. As the name suggests, it suffers from a high time complexity. As depicted in Figure~\ref{fig:system-overview}, static scheduling is invoked as a subroutine for each configuration of $(\{\m{G}_i\}, \{b_i\}, \{\m{D}_i\})$. The high time complexity can be tolerated so far as it leads to optimizing the objective (\ref{opt:objective}), but as explained static scheduling is geared more toward meeting the memory constraint (\ref{opt:constraint}) than optimizing the objective (\ref{opt:objective}). Our empirical experience suggests that optimal schedules demonstrate a particular pattern, thus costly grid search is not necessary. This observation leads us to the next method.

Next, the $k$F$k$B method refers to a scheme that schedules $k$ forward passes followed by $k$ backward passes and repeats this pattern when the pipeline is full. To be concrete, a schedule $\Pi_i$ is said to be $k$F$k$B when there exist $\ell$ and $k$ such that $\Pi_i$ starts with $\ell$ forward passes (for warm-up), alternates between $k$ backward passes and $k$ forward passes, and ends with $\ell$ backward passes (for cool-down). Figure~\ref{fig:1f1b_nfnb}(a) illustrates an $k$F$k$B schedule example where the second stage starts and ends with $\ell = 4$ forward and backward passes respectively, and $k = 2$ backward passes and $k = 2$ forward passes alternate in between. Abiding by this schedule pattern allows us to implement a static scheduling algorithm that reduces the time complexity owing to a much reduced search space.
%followed by $\left( \frac{B}{b_i} - k \right)/n$ cycles, 

Finally, the 1F1B method is a special case of the $k$F$k$B method. In this work, we use 1F1B by default since except for some corner cases where $k$F$k$B outperforms 1F1B, the memory usage performance of 1F1B matches that of $k$F$k$B. Figure~\ref{fig:1f1b_nfnb} illustrates such a corner case. The number of in-flight micro-batches for the first stage is smaller by employing $k$F$k$B for the second stage compared to 1F1B. Note that the micro-batch size for the second stage is half of that for the first and third stages. For the second stage, two backward passes (B1, B2) are scheduled in a row in $k$F$k$B, and a forward pass follows a backward pass (B1, F5) in 1F1B. As a result, the first stage can schedule its backward pass (B1) faster in $k$F$k$B. This helps the first stage resolve an in-flight micro-batch faster, which in turn reduces the number of in-flight micro-batches (hence the reduced activation memory).

Recent work \cite{wang2023ada} investigates performance implications in relatively simpler cases where all stages use the same micro-batch size and employ either 1F1B or $k$F$k$B exclusively, as opposed to our setup where different micro-batch sizes and scheduling methods across distinct stages are allowed. In practice, computations for forward and backward passes take different amounts of time, and so do communications of their results between two stages. Employing $k$F$k$B over 1F1B can enable finer-grained adjustments of these varied computation and communication times to overlap them, hiding the smaller cost of the two. This comes at the expense of increased device memory usage, but can be justified when the execution time saving benefit outweighs the increased memory expense.

On a final note, the idea of using different micro-batch sizes across different stages is similar to the idea of intentional uneven model partitioning in \cite{fan2021dapple} to some extent. The goal is to improve throughput by distributing the workload across stages unevenly and then exploiting heterogeneous compute efficiencies to carry out fine-grained adjustments of stage execution times. The difference is the dimension along which the workload, determined by both the number of data samples to process and the amount of compute operations to execute, is split unevenly. It is along the batch (data samples) dimension in our case, and the model (operations) dimension in \cite{fan2021dapple}.


%Microbatch scheduling generates the schedule strategy $\{\Pi_i\}$ for the input \gpp strategy $\m{G}_s$. Note that microbatch schedule does not affect TPS, so we focus on memory usage here. The optimality of a schedule is therefore defined as:

%\paragraph{Definition (Optimal schedule).} Let $g_{x_1}, g_{x_2}, \ldots, g_{x_{|P|}}$ be a topological order of the stage graph nodes. A schedule $\{\Pi_i\}$ is \textit{optimal} if for any other schedule $\{\Pi'_i\}$ and a stage $x_i$, $\mathrm{inflight}(\Pi'_{x_i}) < \mathrm{inflight}(\Pi_{x_i})$ implies $\mathrm{inflight}(\Pi'_{x_j}) > \mathrm{inflight}(\Pi_{x_j})$ for some $j > i$.

%Our microbatch scheduling algorithm starts from the last stage and generates the schedule for each stage based on its subsequent stages, as described in Algorithm~\ref{alg:microbatch-scheduling}. The appendix introduces an implementation of $\mathrm{ScheduleStrategy}(\cdot) = \mathrm{Greedy}(\cdot)$ that results in a microbatch scheduling algorithm generating an optimal schedule. $\mathrm{Greedy(\cdot)}$ enumerates the number of in-flight microbatches and then tries to schedule each backward microbatch as early as possible. $\mathrm{Greedy(\cdot)}$ takes any arbitrary valid schedules as inputs, and $O(B^2)$ time to derive the schedule for the current stage. In practice, we find that the schedule discovered by the algorithm follows certain patterns. Specifically, most stages periodically process the backward processing of some microbatches followed by the forward processing of the same number of microbatches. We summarize this as nFnB schedule.

%\paragraph{Theorem.} $\mathrm{Greedy}(\cdot)$ gives an optimal schedule.


%\paragraph{nFnB Schedule.} nFnB schedule is a subset of the set of all the valid microbatch schedules for a stage. A valid microbatch schedule $\Pi_i$ for a stage $S_i$ is in nFnB schedule if there exists $i_i$ and $n_i$ such that $\Pi_i$ starts with the forward processing of $i_i$ microbatches, followed by $(B-i_i)/n_i$ cycles, and ends with the backward processing of $i_i$ microbatches, where each cycle is the backward processing of $n_i$ microbatches followed by the forward processing of $n_i$ microbatches. In this case, we also say this stage follows $n_i$F$n_i$B schedule. Figure~\ref{fig:1f1b_nfnb} shows an example where the naive 1F1B schedule leads to higher memory consumption than the nFnB schedule.

%We use $\mathrm{nFnBSchedule}(\cdot)$ as an implementation of $\mathrm{ScheduleStrategy}(\cdot)$ in Algorithm~\ref{alg:microbatch-scheduling}. $\mathrm{nFnBSchedule}(\cdot)$ computes the number of in-flight microbatches under $n_i$F$n_i$B schedule for each possible $n_i$ through a rule-based algorithm (see Appendix), and chooses the $n_i$ that minimizes the number of in-flight microbatches.



==> contents/past_versions/6_scheduler_ver2.tex <==
\section{Static Micro-batch Scheduler}
\label{sec:scheduler}

% \ZJ{The term static scheduler is vague in terms that it doesn't really specify what we are scheduling here. Suggested rename: `Micro-batch Scheduler` or `Static Micro-batch Scheduler`.}

The static micro-batch scheduler ensures correctness of \gpp by meeting the data dependency requirements between all forward and backward passes within a stage (\textit{C4} in \S\ref{sec:gpp}) and those across stages (\textit{C5} in \S\ref{sec:gpp}). Given the stage subgraphs, micro-batch sizes, and device allocations by the pipeline stage partitioner of Algorithm~\ref{alg:faster-partitioner-sp-dp} as input, it produces the micro-batch schedules for all stages as output. Once the micro-batch schedules are determined, the device memory usages that consist of weight and activation memory usages are also determined. Thus, the output of the micro-batch scheduler can indicate whether the device memory constraint of (\ref{opt:constraint}) is met. As shown in \S\ref{sec:partitioner}, we use the micro-batch scheduler, to be described in Algorithm~\ref{alg:microbatch-scheduling}, as a key subroutine of Algorithm~\ref{alg:faster-partitioner-sp-dp}.

\begin{algorithm}[th!]
	\small
	\caption{Static Micro-batch Scheduler} \label{alg:microbatch-scheduling}
	\textbf{Input}: Stage subgraphs $\{\m{G}_i\}$, micro-batch sizes $\{b_i\}$, device allocations $\{\m{D}_i\}$ \\
	\textbf{Output}: Schedules $\{\Pi_i\}$\\
	\begin{algorithmic}[1]
            \For {$S_i \in \m{V}_S$}
                \If {no micro-batch schedule is specified for $S_i$}
                    \State \Call{ScheduleStages}{$S_i$}
                \EndIf
            \EndFor
            \Function{ScheduleStages}{$S_i$}
                \For {$(S_i, S_j) \in \m{E}_S$}
                    \If {no micro-batch schedule is specified for $S_j$}
                        \State \Call{ScheduleStages}{$S_j$}
                    \EndIf
                \EndFor
                \State $\Pi_i \gets$ \Call{ScheduleTasks}{$b_i, \m{D}_i, \{\Pi_j \mid (S_i, S_j) \in \m{E}_S\}$}
            \EndFunction
	\end{algorithmic}
\end{algorithm}

% Algorithm~\ref{alg:microbatch-scheduling} describes static scheduling in detail.
As input, the micro-batch scheduler takes a configuration of model partition $\{ \m{G}_i \}$, micro-batch sizes $\{ b_i \}$, and device assignment $\{ \m{D}_i \}$. As output, it produces the set of static micro-batch schedules $\{ \Pi_i \}$ of all forward and backward passes for all stages. As shown in Figure~\ref{fig:system-overview}, the input is fed by the stage partitioner, and the output is returned back to it to indicate feasibility of the input.

Function \textsf{ScheduleStages} in Algorithm~\ref{alg:microbatch-scheduling} performs recursive search over stage graph $\m{G}_S = (\m{V}_S, \m{E}_S)$. It starts by first specifying a schedule for the last stage. Then for $(S_i, S_j) \in \m{E}_S$, it traces back the directed edges in $\m{E}_S$ of $\m{G}_S$ in reverse and specifies schedules for stages $S_i$ until a schedule for the first stage is finally specified. The reason for backward traversal is that computing the activation memory usage, and thus the total usage, for a stage $S_i$ requires complete schedule information of subsequent stages $S_j$ for $(S_i, S_j) \in \m{E}_S$.

Function \textsf{ScheduleTasks} in Algorithm~\ref{alg:microbatch-scheduling} specifies a schedule of all forward and backward tasks within a stage. Combined with \textsf{ScheduleStages}, it ensures the data dependency requirements \textit{C4--C5} in \S\ref{sec:gpp}. 

% \ZJ{FIXME: We didn't define the three methods before.}
% \SOO{We will work on rewriting this section in general and let you know}
In scheduling forward and backward passes within a stage, there exist three methods: exhaustive, 1F1B, and $k$F$k$B.

First, as the name suggests, the exhaustive method performs exhaustive search to find the best micro-batch sizes for all stages. 
It also attempts to schedule each backward pass as early as possible within a stage in order to resolve in-flight micro-batches fast. We prove that the greedy method produces an optimal schedule, and defer the proof and the details of the implementation to Appendix~\ref{sec:greedy-proof}.

As the name suggests, the greedy scheduling algorithm suffers from a high time complexity. As depicted in Figure~\ref{fig:system-overview}, static scheduling is invoked as a subroutine for each configuration of $(\{\m{G}_i\}, \{b_i\}, \{\m{D}_i\})$. Thus, it is desirable to curb its high time complexity.
% is can be tolerated so far as it helps optimize the objective (\ref{opt:objective}). But as explained, static scheduling is geared more toward meeting the memory constraint (\ref{opt:constraint}).
Our empirical experience suggests that optimal schedules demonstrate a particular pattern, thus costly grid search is not necessary in practice. This observation leads us to the next method.

Next, the 1F1B method is a special case of $k$F$k$B (i.e., $k=1$). We employ 1F1B by default in this work. Except for some corner cases where $k$F$k$B outperforms 1F1B, their memory usages are identical. Figure~\ref{fig:1f1b_nfnb} illustrates such a corner case. The number of in-flight micro-batches for the first stage is smaller by $k$F$k$B for the second stage compared to 1F1B. Note that the micro-batch size for the second stage is half of that for the first and third stages. For the second stage, two backward passes (B1, B2) are scheduled in a row in $k$F$k$B, and a forward pass follows a backward pass (B1, F5) in 1F1B. As a result, the first stage can schedule its backward pass (B1) faster in $k$F$k$B, which enables it to resolve an in-flight micro-batch faster and reduce the number of in-flight micro-batches.

Finally, the $k$F$k$B method refers to a scheme that schedules $k$ forward passes followed by $k$ backward passes and repeats this pattern when the pipeline is full.\footnote{To be concrete, a schedule $\Pi_i$ is said to be $k$F$k$B when there exist $\ell$ and $k$ such that $\Pi_i$ starts with $\ell$ forward passes (for warm-up), alternates between $k$ backward passes and $k$ forward passes, and ends with $\ell$ backward passes (for cool-down).} Figure~\ref{fig:1f1b_nfnb}(a) illustrates an $k$F$k$B schedule.
% example where the second stage starts and ends with $\ell = 4$ forward and backward passes respectively, and $k = 2$ backward passes and $k = 2$ forward passes alternate in between.
This simple pattern allows us to implement a static scheduling algorithm that reduces the time complexity owing to a much reduced search space. See Appendix~\ref{sec:nfnbrule}.
%followed by $\left( \frac{B}{b_i} - k \right)/n$ cycles, 


\begin{figure}
    \centering
    \includegraphics[width=\columnwidth]{fig/1F1BvsnFnB.pdf}
    \caption{A comparison between 1F1B and more general $k$F$k$B schedules when stages have different micro-batch sizes. F$\{i,j\}$, B$\{i,j\}$ means forward and backward pass for micro-batch including sample $i$ and $j$. It showcases how $k$F$k$B can be better than 1F1B in terms of memory footprint.}
    \label{fig:1f1b_nfnb}
\end{figure}


\paragraph{Static Scheduling Performance.} In evaluating the performances of different micro-batch schedules, we can take memory usage or time complexity standpoints. Let us focus on the memory usage criterion, as static scheduling is not directly related to the objective  (\ref{opt:objective}) of the optimization problem, but rather closely-related to the memory constraint (\ref{opt:constraint}). Also, whenever we discuss performance, we can reason about its \emph{optimality} aspect. In words, a schedule can be said optimal in terms of memory usage when no other schedule can achieve a better memory usage pattern. The formal definition is as follows.

\begin{definition}[Optimal Schedule] Let $S_1, \dots, S_{|\m{V}_S|}$ be a topological order of stages in $\m{V}_S$. A schedule $\{\Pi_i\}$ is optimal if for any other schedule $\{\Pi'_i\}$ and a stage $S_i$, $\textsf{in-flight}(\Pi'_i) < \textsf{in-flight}(\Pi_i)$ implies $\textsf{in-flight}(\Pi'_j) > \textsf{in-flight}(\Pi_j)$ for some $j > i$, where $\textsf{in-flight}(\Pi_i)$ is the maximum number of in-flight micro-batches for stage $S_i$ at some moment according to $\Pi_i$.
\end{definition}

Recent work \cite{wang2023ada} explores performance implications in cases where all stages use the same micro-batch size and employ either 1F1B or $k$F$k$B exclusively. In contrast, our setup allows where different micro-batch sizes and scheduling methods across distinct stages. In practice, computations for forward and backward passes take different amounts of time, and so do communications of their results. Thus, employing $k$F$k$B over 1F1B can enable finer-grained adjustments of these varied computation and communication times to overlap them, hiding the smaller cost. This comes at the expense of increased device memory usage, but can be justified when the execution time saving benefit outweighs it.

On a final note, the idea of using different micro-batch sizes across different stages is to some extent similar to the idea of intentional uneven model partitioning in recent work \cite{fan2021dapple}. The shared goal is to improve throughput by distributing workloads across stages unevenly and then exploiting heterogeneous compute efficiencies to carry out fine-grained adjustments of stage execution times. The difference is the dimension along which the workloadsare split unevenly. It is along the batch (data samples) dimension in our work, and the model (operations) dimension in \cite{fan2021dapple}.
% , determined by both the number of data samples to process and the amount of compute operations to execute, 

==> contents/past_versions/8_related_ver1.tex <==
\section{Related Work}
\label{sec:related}

% Add automated parallelism works

\paragraph{Data parallelism.} Data parallelism \cite{valiant1990bridging, krizhevsky2014one, li2014scaling, goyal2017accurate} is one of parallel DNN training techniques in which  every device has a local copy of a DNN to train in its entirety and a batch of training data is split across devices. Each device updates its model parameters based on its share of training data and synchronizes the parameters periodically with other devices. In our work, we apply data parallelism within a pipeline stage to which we assign multiple devices, in order to balance stage execution times in a more fine-grained manner compared to applying pipeline parallelism only.

\paragraph{Model parallelism.} Model parallelism is another technique in which the the DNN is split across devices instead of the data batch. Each device executes and performs updates for only a subset of the model parameters.  An individual operator (such as matrix multiplication) can be sliced across devices as in \cite{shoeybi2019megatron, zheng2022alpa}. Alternatively, groups of operators are distributed across devices as in pipeline parallelism.

\paragraph{Synchronous pipeline parallelism.} Synchronous pipeline parallelism \cite{huang2019gpipe, narayanan2021memory, fan2021dapple, zheng2022alpa} refers to a set of techniques in which the model parameters spread across devices are updated synchronously after each batch is processed in one training iteration. The DNN training semantics is preserved, thus statistical convergence issues do not arise. But the synchronous parameter update mechanism fills and drains the pipeline periodically over iterations hurting training throughput. Graph pipeline parallelism mitigates this issue by reducing pipeline bubbles better than sequential pipeline parallelism.

% GPipe \cite{huang2019gpipe} investigates synchronous pipeline parallel training for the first time in distributed DNN training. GPipe takes as input a DNN model partitioned into $K$ sequential segments, assignes each to one of $K$ devices, and splits a batch into $M$ micro-batches. Each device processes a forward pass of $M$ micro-batches and a corresponding backward pass, passing a completed micro-batch onto the next device in the pipeline. As specific details as to how GPipe carries out batch splitting are left out, we consider other subsequent approaches that develop automated algorithms to realize synchronous pipeline parallel training as our primary baselines.

% Concurrent work PipeDream-Flush \cite{narayanan2021memory} and DAPPLE \cite{fan2021dapple} also employ the synchronous pipeline as with GPipe, but they feature additional key techniques aimed to reduce device memory usage. In PipeDream-Flush, each device alternates between forward and backward passes $M$ times to process the $M$ micro-batches. This 1F1B schedule keeps low memory footprint over GPipe by limiting activation stashes to in-flight micro-batches only. DAPPLE injects $K (< M)$ micro-batches and schedules backward passes as early as possible, which also realizes the 1F1B schedule while the pipeline is full.

% Compared to the aforementioned work, Alpa \cite{zheng2022alpa} additionally employs tensor-parallelization techniques where tensors associated with operators are split and processed across multiple devices. Alpa proposes an automated algorithm that explores the augmented search space efficiently to devise a training strategy that combines pipeline parallelism with tensor- and data-parallelization techniques.

\paragraph{Asynchronous pipeline parallelism.} Asynchronous pipeline parallelism \cite{narayanan2019pipedream, narayanan2021memory, tarnawski2021piper,wpipe} refers to a set of techniques in which the model parameters spread across devices are updated asynchronously. Although this mode may suffer from statistical convergence issues as devices execute their stages using out-of-sync model parameters, it keeps the pipeline full at nearly all times. Graph pipeline parallelism helps us reduce total device memory usage, thus use a larger micro-batch size to execute operators at a higher operational intensity compared to sequential pipeline parallelism. This enables us to process training data faster while the pipeline is full, thus improves training throughput.

% PipeDream \cite{narayanan2019pipedream} investigates asynchronous pipeline parallel training for the first time in distributed DNN training and subsequent work PipeDream-2BW \cite{narayanan2021memory} improves upon PipeDream by employing double-buffered weight updates to reduce device memory usage. Both adopt the 1F1B schedule.

% Piper \cite{tarnawski2021piper} develops an automated algorithm that combines pipeline parallelism with tensor- and data-parallel techniques to devise a strategy that minimizes the latency of the bottleneck pipeline stage under the 1F1B schedule in asynchronous pipeline-parallel training. Piper assumes a handful of good tensor-parallel techniques are already available for some number of layers to make it tractable to explore the search space of parallelization technique combinations.

\paragraph{Multiple pipeline stages per device.} In the above pipeline-parallel techniques, each device contains only one pipeline stage. It has been shown that assigning multiple non-contiguous stages to a device can reduce pipeline bubbles \cite{narayanan2021efficient, lamy2022breadth} and reduces memory consumption imbalances across stages~\cite{li2021chimera, hanayo}. Earlier work GEMS~\cite{gems} has a similar idea but failed to utilize the pipeline well -- devices are idle for most of the time and waiting for results from other stages. These techniques are orthogonal to graph pipeline parallelism, and thus may be applicable upon some modifications.
%Consider a simple four-layer DNN and two devices. One can assign layers 1, 2 to device A and layers 3, 4 to device B. Instead, one can assign layers 1, 3 to device A and layers 2, 4 to device B. In the former, the pipeline bubble at the beginning of each iteration is device A's execution time for layers 1 and 2, after which device B starts processing its share. In the latter, it is device A's execution time for layer 1.

\paragraph{Memory optimizations.}  Managing memory usage patterns is critical in training large DNNs. Thus, on top of pipeline-parallel techniques, memory optimization techniques \cite{chen2016training, rhu2016vdnn, wang2018superneurons, zhang2019efficient, choukse2020buddy, peng2020capuchin, huang2020swapadvisor, jain2020checkmate, ren2021zero, chen2021actnn} can also be modified and applied in order to further improve the performance and scalability of graph pipeline parallelism.

% \paragraph{Key Technical Distinction.} We develop \emph{graph-like} pipeline parallelism for the first time in distributed DNN training, where multiple independent stages can process the same micro-batch concurrently. It also allows for using different micro-batch sizes for different stages, which can lead to higher throughput by leveraging heterogeneities across pipeline stages. Moreover, unlike nearly all existing approaches that strictly adhere to the 1F1B schedule, our approach explores the general $k$F$k$B schedule that can lead to lower device memory usage and higher training throughput.
% This benefit of employing nFnB over 1F1B has been illustrated in Figure.~\ref{fig:nFnB-1F1B}. 

% Let us discuss the theoretical possibility that extending some existing approaches can find a training strategy idential to ours. For instance, one could argue that extending \cite{zheng2022alpa} achieves the same partitioning capability as ours. After having a pipeline stage partition in place, one could explore model-parallel techniques within a single stage to further split that stage into multiple independent \emph{sub}stages that can process the same micro-batch concurrently. This extension greatly complicates the integer linear programming part of \cite{zheng2022alpa} where compute, communication, resharding costs must be evaluated for all operators and all edges between the operators. To make the extension work, such costs must be evaluated for all \emph{combinations} of operator groups and all edges between the groups. This highlights the novelty of our approach that expands the search space for pipeline-parallel training strategies, yet efficiently finds a high-performant one.

% \textbf{Automated parallelism.} Alpa, Unity, FlexFlow

% \textbf{Pipeline parallelism.}

% \textbf{Model parallelism.}

% \textbf{Data parallelism.}

% \textbf{Activation recomputation.} Our approach is orthogonal to recomputation approaches.jb

==> contents/past_versions/outdated.tex <==
\section{Evaluation}
\label{sec:evaluation}

\subsection{Implementation and Experimental Setup}
Hardware: 64 A100 (or V100) GPUs \\ \\ 
\textbf{Models}
\begin{outline}[enumerate]
\1 Image - text (e.g., CLIP, ALIGN)
    \2 Balanced (two Transformers)
    \2 Unbalanced (ResNet + Transformer)
\1 Image - image (e.g., RGB + Optical flow)
\1 Candle-Uno
\1 DLRM 
\end{outline}
\textbf{Baselines}
\begin{outline}[enumerate]
\1 Linear pipeline
\end{outline}

\subsection{End-to-end Evaluation}
Weak scaling plot \\ 
- X-axis: Number of devices (4, 8, 16, 32, 64) \\
- Y-axis: Throughput (samples / second) \\
\begin{outline}[enumerate]
\1 Image - text (e.g., CLIP, ALIGN)
    \2 Balanced (two Transformers)
    \2 Unbalanced (ResNet + Transformer)
\1 Image - image (e.g., RGB + Optical flow)
\1 Candle-Uno
\1 DLRM 
\end{outline}

\subsection{Search Time}
Table \\ 
- X-axis: Number of devices (4, 8, 16, 32, 64) \\
- Y-axis: Search time (sec) with/without our techniques to reduce search time\\
Refer to Unity paper

\begin{figure*}[htbp]
	\centering
	\subfigure[2stream-config1]{\includegraphics[width=0.24\textwidth]{fig/exp/throughput-2stream.png}\label{2stream}}
	\subfigure[2stream-config2 ]{\includegraphics[width=0.24\textwidth]{fig/exp/throughput-cs2_2.png}\label{cs2-2}}
	\subfigure[2stream-config3 ]{\includegraphics[width=0.24\textwidth]{fig/exp/throughput-cs2_3.png}\label{cs2-3}}
        \subfigure[Candle-Uno ]
    {\includegraphics[width=0.24\textwidth]{fig/exp/throughput-candle.png}\label{candle-uno}}
	\caption{End-to-end Performance}
	\label{fig:e2e}
\end{figure*}
\subsection{Minibatch Size}
\begin{figure*}[htbp]
	\centering
	\subfigure[2stream-config1(nd=8)]{\includegraphics[width=0.24\textwidth]{fig/exp/2stream.pdf}\label{2stream-mb}}
	\subfigure[2stream-config2(nd=8) ]{\includegraphics[width=0.24\textwidth]{fig/exp/cs2-2.pdf}\label{cs2-2-mb}}
	\subfigure[2stream-config3(nd=8) ]{\includegraphics[width=0.24\textwidth]{fig/exp/cs2-3.pdf}\label{cs2-3-mb}}
     \subfigure[2stream-config1(nd=4) ]{\includegraphics[width=0.24\textwidth]{fig/exp/2stream-nd4.pdf}\label{cs2-3-mb}}
	\caption{Throughput with different minibatch size.}
	\label{fig:mb}
\end{figure*}
% small minibatch size
\subsection{Workload Balance}
% a table showing num of attention op for each stage
\begin{figure}
    \centering
    \includegraphics[width=0.4\textwidth]{fig/exp/cs4-1.pdf}
    \caption{Memory Pressure Test. (GPP with more balanced workload)}
    \label{fig:cs4-1}
\end{figure}

\subsection{More Branches}
% synthetic 4-2 4-3
\begin{figure}[htbp]
	\centering
	\subfigure[4stream-config2]{\includegraphics[width=0.23\textwidth]{fig/exp/throughput-cs4-2.png}\label{cs4-2}}
	\subfigure[4stream-config3 ]{\includegraphics[width=0.23\textwidth]{fig/exp/throughput-cs4-3.png}\label{cs4-3}}
	\caption{4-Stream Cases}
	\label{fig:4stream}
\end{figure}

